Region growing for multi-route cuts

We study a number of multi-route cut problems: given a graph G=(V,E) and connectivity thresholds k_(u,v) on pairs of nodes, the goal is to find a minimum cost set of edges or vertices the removal of which reduces the connectivity between every pair (u,v) to strictly below its given threshold. These problems arise in the context of reliability in communication networks; They are natural generalizations of traditional minimum cut problems where the thresholds are either 1 (we want to completely separate the pair) or infinity (we don't care about the connectivity for the pair). We provide the first non-trivial approximations to a number of variants of the problem including for both node-disjoint and edge-disjoint connectivity thresholds. A main contribution of our work is an extension of the region growing technique for approximating minimum multicuts to the multi-route setting. When the connectivity thresholds are either 2 or infinity (the "2-route cut" case), we obtain polylogarithmic approximations while satisfying the thresholds exactly. For arbitrary connectivity thresholds this approach leads to bicriteria approximations where we approximately satisfy the thresholds and approximately minimize the cost. We present a number of different algorithms achieving different cost-connectivity tradeoffs.

==> abstract.tex <==
We study a number of \emph{multi-route cut} problems: given a graph
$G=(V,E)$ and connectivity thresholds $k_{(u,v)}$ on pairs of nodes,
the goal is to find a minimum cost set of edges or vertices the
removal of which reduces the connectivity between every pair $(u,v)$
to strictly below its given threshold. These problems arise in the
context of reliability in communication networks; They are natural
generalizations of traditional minimum cut problems where the
thresholds are either $1$ (we want to completely separate the pair) or
$\infty$ (we don't care about the connectivity for the pair). We
provide the first non-trivial approximations to a number of variants
of the problem including for both node-disjoint and edge-disjoint
connectivity thresholds. A main contribution of our work is an
extension of the region growing technique for approximating minimum
multicuts to the multi-route setting. When the connectivity thresholds
are either $2$ or $\infty$ (the ``$2$-route cut'' case), we obtain
polylogarithmic approximations while satisfying the thresholds
exactly. For arbitrary connectivity thresholds this approach leads to
bicriteria approximations where we approximately satisfy the
thresholds and approximately minimize the cost. We present a number of
different algorithms achieving different cost-connectivity tradeoffs.

%we present a version of
%the region growing lemma where the thresholds are violated by a factor
%of at most $2$.
